A Note on the Modeling Power of Different Graph Types

Graphs can have different properties that lead to several graph types and may allow for a varying representation of diverse information. In order to clarify the modeling power of graphs, we introduce a partial order on the most common graph types based on an expressivity relation. The expressivity relation quantifies how many properties a graph type can encode compared to another type. Additionally, we show that all attributed graph types are equally expressive and have the same modeling power.

==> chapters/notation.tex <==
\section{Notation}\label{sec_Notation}
%\begin{longtable}{|>{\centering}p{0.45\textwidth}|>{\centering}p{0.45\textwidth}|}
%	\hline
%	 $\mathbb{N}$ & natural numbers $\{1,2,\ldots\}$\\
%	 $\mathbb{N}_0$ & natural numbers beginning at $0: \{0,1,\ldots\}$\\
%	 \hline
%\end{longtable}
\textcolor{red}{Die Tabelle muss man natürlich nochmal anpassen...}

\begin{table}
  \centering
  \begin{tabular}{|l|l|}
    \hline
    $\mathbb{N}$ & natural numbers\\
    $\mathbb{N}_0$ & natural numbers starting at $0$\\
    \hline
    $|\cdot|$ & absolute value \\
    $[n], \,n\in \mathbb{N}$ & sequence $1,2,\ldots, n$ \\
    $[n]_{0}, \,n\in \mathbb{N}_{0}$ & sequence $0,1,\ldots, n$ \\
    \hline
    $\emptyset$ & empty set\\
    $\{\cdot\}$ & set \\
    $\{\cdot\}^*$ &  tuple of arbitrary length over $\{\cdot\}$\\
    $\{\!\vert\cdot\vert\!\}$ & multiset, i.e. set allowing multiple appearances of entries\\
    $\set{P}(\cdot)$ & power (multi)set\\
    \hline
    $\wedge$ & conjunction \\ 
    $\cup$ & union of two (multi)sets\\
    $\cupdot$ & disjoint union of two (multi)sets \\
    $\subseteq$ & sub(multi)set \\
    $\subset$ & proper sub(multi)set \\
    $\times $ & factor set of two sets\\
    \hline
    $[\cdot,\ldots,\cdot]$ & listing \\
    $[\cdot,\ldots,\cdot\mid \cdot]$ & list comprehension \\
    \hline
  \end{tabular}
  \caption{Notation table\label{notationtable}}
\end{table}

% \section{Limited Embedding of Attributed Graph Types into Unattributed Graphs}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../mog"
%%% End:
